Shape and Spectrum: On the Heat and Volume of Self-Similar Fractals

In this work, we examine the relationship between geometry and spectrum of regions with fractal boundary. The relationship is well-understood for fractal harps in one dimension, but largely open for fractal drums in larger dimensions. To that end, we study fractals arising as attractors of self-similar iterated function systems with some separation conditions. On the geometric side, we analyze the tube zeta functions and their poles, called complex dimensions, which govern the asymptotics of the volume of tubular neighborhoods of such fractals. On the spectral side, we study a Dirichlet problem for the heat equation, closely related to spectrum of the Laplacian. We show that the asymptotics of the total heat content are controlled by the same set of possible complex dimensions. Our method is to establish scaling functional equations and to solve by means of truncated Mellin transforms, wherefrom the scaling ratios of the underlying dynamics can be seen to govern both the geometry and spectra of these self-similar fractal drums.

==> commands/_thmSetupTCB.tex <==
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%
%           ██╗    ██╗██╗██╗     ██╗         ██╗  ██╗ ██████╗ ███████╗███████╗███████╗██████╗
%           ██║    ██║██║██║     ██║         ██║  ██║██╔═══██╗██╔════╝██╔════╝██╔════╝██╔══██╗
%           ██║ █╗ ██║██║██║     ██║         ███████║██║   ██║█████╗  █████╗  █████╗  ██████╔╝
%           ██║███╗██║██║██║     ██║         ██╔══██║██║   ██║██╔══╝  ██╔══╝  ██╔══╝  ██╔══██╗
%           ╚███╔███╔╝██║███████╗███████╗    ██║  ██║╚██████╔╝██║     ██║     ███████╗██║  ██║
%            ╚══╝╚══╝ ╚═╝╚══════╝╚══════╝    ╚═╝  ╚═╝ ╚═════╝ ╚═╝     ╚═╝     ╚══════╝╚═╝  ╚═╝
%
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
\RequirePackage{tcolorbox}
\tcbuselibrary{skins}

% Theorems counter
\newcounter{theo}[section]
\numberwithin{theo}{section}

% TColorBox Style
\newtcolorbox{mybox}[1]{
    colback=blue!5,
    colbacktitle=blue!20,
    coltitle=black,
    colframe=blue,
    fonttitle=\bfseries,
    title={#1},
    enhanced,
    attach boxed title to top text left={xshift=0mm,yshift=-2mm},
    boxed title style={arc=0mm},
    arc=0mm,
}

% General environment setup
\newcommand{\envSetup}[2]{
    \newenvironment{#1}[1][]
    {%
        \refstepcounter{theo}%
        \begin{mybox}{\strut #2~\thetheo\ifstrempty{##1}{}{:~##1}}\relax%
    }
    {\end{mybox}}
}

% Create the environments for theorems, lemmas, etc.
\envSetup{theorem}{Theorem}
\envSetup{definition}{Definition}
\envSetup{lemma}{Lemma}
\envSetup{proposition}{Proposition}
\envSetup{corollary}{Corollary}
\envSetup{assumption}{Assumption}
\envSetup{myAbstract}{Abstract}

% Allow or disallow frames to split across page breaks
% \mdfsetup{nobreak=true}
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%█..............................................................................................................█
%█................................................................................**............................█
%█...........................................................................***********........................█
%█..........................................................................************........................█
%█............................................................................*********.........................█
%█..................................................................*....*.************..*......................█
%█..........................................................*****..*.**************************.................█
%█..........................................................***************************************.*****.......█
%█...........................................................*******************************************........█
%█.....................................................***.********************************************.*.......█
%█.......................................................*************************************************......█
%█..................................................********************************************************....█
%█...................................................*****************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...........................*****************.....*******************************************************......█
%█........................***********************.*********************************************************.....█
%█........................***********************.********************************************************......█
%█..................****.********************************************************************************.......█
%█**************************************************************************************************............█
%█..................****.********************************************************************************.......█
%█........................***********************.********************************************************......█
%█........................***********************.*********************************************************.....█
%█...........................*****************.....*******************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...................................................*****************************************************......█
%█..................................................********************************************************....█
%█......................................................*************************************************.......█
%█....................................................***.********************************************.*........█
%█..........................................................*******************************************.........█
%█.........................................................***************************************.*****........█
%█.........................................................*****..*.**************************..................█
%█.................................................................*....*.************..*.......................█
%█...........................................................................*********..........................█
%█.........................................................................************.........................█
%█..........................................................................***********.........................█
%█...............................................................................**.............................█
%█..............................................................................................................█
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

==> commands/letterCommands.tex <==
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%
%           ██╗    ██╗██╗██╗     ██╗         ██╗  ██╗ ██████╗ ███████╗███████╗███████╗██████╗
%           ██║    ██║██║██║     ██║         ██║  ██║██╔═══██╗██╔════╝██╔════╝██╔════╝██╔══██╗
%           ██║ █╗ ██║██║██║     ██║         ███████║██║   ██║█████╗  █████╗  █████╗  ██████╔╝
%           ██║███╗██║██║██║     ██║         ██╔══██║██║   ██║██╔══╝  ██╔══╝  ██╔══╝  ██╔══██╗
%           ╚███╔███╔╝██║███████╗███████╗    ██║  ██║╚██████╔╝██║     ██║     ███████╗██║  ██║
%            ╚══╝╚══╝ ╚═╝╚══════╝╚══════╝    ╚═╝  ╚═╝ ╚═════╝ ╚═╝     ╚═╝     ╚══════╝╚═╝  ╚═╝
%
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

%----------------------------------------------------------------------------------------------------------------
% Math Blackboard Bold
\providecommand{\AA}{\mathbb{A}}
\providecommand{\BB}{\mathbb{B}}
\providecommand{\CC}{\mathbb{C}}
\providecommand{\DD}{\mathbb{D}}
\providecommand{\EE}{\mathbb{E}}
\providecommand{\FF}{\mathbb{F}}
\providecommand{\GG}{\mathbb{G}}
\providecommand{\HH}{\mathbb{H}}
\providecommand{\II}{\mathbb{I}}
\providecommand{\JJ}{\mathbb{J}}
\providecommand{\KK}{\mathbb{K}}
\providecommand{\LL}{\mathbb{L}}
\providecommand{\MM}{\mathbb{M}}
\providecommand{\NN}{\mathbb{N}}
\providecommand{\OO}{\mathbb{O}}
\providecommand{\PP}{\mathbb{P}}
\providecommand{\QQ}{\mathbb{Q}}
\providecommand{\RR}{\mathbb{R}}
\providecommand{\SS}{\mathbb{S}}
\providecommand{\TT}{\mathbb{T}}
\providecommand{\UU}{\mathbb{U}}
\providecommand{\VV}{\mathbb{V}}
\providecommand{\WW}{\mathbb{W}}
\providecommand{\XX}{\mathbb{X}}
\providecommand{\YY}{\mathbb{Y}}
\providecommand{\ZZ}{\mathbb{Z}}

%----------------------------------------------------------------------------------------------------------------
% Math Embellished Script
\providecommand{\A}{\mathscr{A}}
\providecommand{\B}{\mathscr{B}}
\providecommand{\C}{\mathscr{C}}
\providecommand{\D}{\mathscr{D}}
\providecommand{\E}{\mathscr{E}}
\providecommand{\F}{\mathscr{F}}
\providecommand{\G}{\mathscr{G}}
\providecommand{\H}{\mathscr{H}}
\providecommand{\I}{\mathscr{I}}
\providecommand{\J}{\mathscr{J}}
\providecommand{\K}{\mathscr{K}}
\providecommand{\L}{\mathscr{L}}
\renewcommand{\L}{\mathscr{L}}
\providecommand{\M}{\mathscr{M}}
\providecommand{\N}{\mathscr{N}}
\providecommand{\O}{\mathscr{O}}
\providecommand{\P}{\mathscr{P}}
\renewcommand{\P}{\mathscr{P}}
\providecommand{\Q}{\mathscr{Q}}
\providecommand{\R}{\mathscr{R}}
\providecommand{\S}{\mathscr{S}}
\providecommand{\T}{\mathscr{T}}
\providecommand{\U}{\mathscr{U}}
\providecommand{\V}{\mathscr{V}}
\providecommand{\W}{\mathscr{W}}
\providecommand{\X}{\mathscr{X}}
\providecommand{\Y}{\mathscr{Y}}
\providecommand{\Z}{\mathscr{Z}}

%----------------------------------------------------------------------------------------------------------------
% Math Caligraphic Script
\providecommand{\Aa}{\mathcal{A}}
\providecommand{\Bb}{\mathcal{B}}
\providecommand{\Cc}{\mathcal{C}}
\providecommand{\Dd}{\mathcal{D}}
\providecommand{\Ee}{\mathcal{E}}
\providecommand{\Ff}{\mathcal{F}}
\providecommand{\Gg}{\mathcal{G}}
\providecommand{\Hh}{\mathcal{H}}
\providecommand{\Ii}{\mathcal{I}}
\providecommand{\Jj}{\mathcal{J}}
\providecommand{\Kk}{\mathcal{K}}
\providecommand{\Ll}{\mathcal{L}}
\providecommand{\Mm}{\mathcal{M}}
\providecommand{\Nn}{\mathcal{N}}
\providecommand{\Oo}{\mathcal{O}}
\providecommand{\Pp}{\mathcal{P}}
\providecommand{\Qq}{\mathcal{Q}}
\providecommand{\Rr}{\mathcal{R}}
\providecommand{\Ss}{\mathcal{S}}
\providecommand{\Tt}{\mathcal{T}}
\providecommand{\Uu}{\mathcal{U}}
\providecommand{\Vv}{\mathcal{V}}
\providecommand{\Ww}{\mathcal{W}}
\providecommand{\Xx}{\mathcal{X}}
\providecommand{\Yy}{\mathcal{Y}}
\providecommand{\Zz}{\mathcal{Z}}

% Greek Letter Shortcuts
\providecommand{\ph}{\varphi}


% -------------------------------------------------------------------------------------------------
% Command Renewal 
% -------------------------------------------------------------------------------------------------
% This overwrites commands that exist elsewhere (usually prebuilt accent commands.) 
% Include this file last if you need to overwrite commands from other packages 
% (and potentially if you encounter issues)
% -------------------------------------------------------------------------------------------------
\renewcommand{\H}{\mathscr{H}}


%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%█..............................................................................................................█
%█................................................................................**............................█
%█...........................................................................***********........................█
%█..........................................................................************........................█
%█............................................................................*********.........................█
%█..................................................................*....*.************..*......................█
%█..........................................................*****..*.**************************.................█
%█..........................................................***************************************.*****.......█
%█...........................................................*******************************************........█
%█.....................................................***.********************************************.*.......█
%█.......................................................*************************************************......█
%█..................................................********************************************************....█
%█...................................................*****************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...........................*****************.....*******************************************************......█
%█........................***********************.*********************************************************.....█
%█........................***********************.********************************************************......█
%█..................****.********************************************************************************.......█
%█**************************************************************************************************............█
%█..................****.********************************************************************************.......█
%█........................***********************.********************************************************......█
%█........................***********************.*********************************************************.....█
%█...........................*****************.....*******************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...................................................*****************************************************......█
%█..................................................********************************************************....█
%█......................................................*************************************************.......█
%█....................................................***.********************************************.*........█
%█..........................................................*******************************************.........█
%█.........................................................***************************************.*****........█
%█.........................................................*****..*.**************************..................█
%█.................................................................*....*.************..*.......................█
%█...........................................................................*********..........................█
%█.........................................................................************.........................█
%█..........................................................................***********.........................█
%█...............................................................................**.............................█
%█..............................................................................................................█
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

==> commands/notation.tex <==
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%
%           ██╗    ██╗██╗██╗     ██╗         ██╗  ██╗ ██████╗ ███████╗███████╗███████╗██████╗
%           ██║    ██║██║██║     ██║         ██║  ██║██╔═══██╗██╔════╝██╔════╝██╔════╝██╔══██╗
%           ██║ █╗ ██║██║██║     ██║         ███████║██║   ██║█████╗  █████╗  █████╗  ██████╔╝
%           ██║███╗██║██║██║     ██║         ██╔══██║██║   ██║██╔══╝  ██╔══╝  ██╔══╝  ██╔══██╗
%           ╚███╔███╔╝██║███████╗███████╗    ██║  ██║╚██████╔╝██║     ██║     ███████╗██║  ██║
%            ╚══╝╚══╝ ╚═╝╚══════╝╚══════╝    ╚═╝  ╚═╝ ╚═════╝ ╚═╝     ╚═╝     ╚══════╝╚═╝  ╚═╝
%
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

\RequirePackage{mathtools}

%----------------------------------------------------------------------------------------------------------------
% Notation Macros
\providecommand{\Laplace}{\mathcal{L}}
\providecommand{\Fourier}{\mathcal{F}}
\providecommand{\Borel}{\mathcal{B}}
\providecommand{\Mellin}{\mathcal{M}}
\providecommand{\CMSpace}{\mathbb{C}\mathbb{M}}
\providecommand{\LCMSpace}{\mathbb{C}\mathbb{M}_{\text{loc}}}
\providecommand{\Somega}{\widetilde S_\Omega}
\providecommand{\testfn}{\psi}
\providecommand{\simdim}{\dim_S}
\providecommand{\lowersimdim}{\underline{\dim}_S}

\providecommand{\xilf}{\xi_{L,f}}
\providecommand{\xilfphi}{\xi_{\Phi,f}}
\providecommand{\xilfphia}{\xi_{L_\Phi^\alpha,f}}

% Heat Content
\newcommand{\Region}{\Omega}
\newcommand{\Regionbd}{X}
\newcommand{\Regionplus}{Y}
\newcommand{\heatContent}{E_\Region}
\newcommand{\heatzeta}{\widehat{\zeta}_{\Region}}
\newcommand{\partialheatzeta}{\widehat{\xi}_\Region}
\newcommand{\genheatzeta}{\widehat{\zeta}_{\Region,F}}
\newcommand{\rempow}{{(\dimension-\sigma_0)}}
\newcommand{\remset}{{\Omega_R}}
\DeclarePairedDelimiter{\bracket}{\langle}{\rangle}
\newcommand{\frem}{f_{\text{Rem}}}
\newcommand{\heatop}{\Hh}
\DeclareMathOperator{\Mean}{\text{Mean}}
\newcommand{\heatmean}{\mathscr{M}}
\newcommand{\decompRem}{R_\Region}

\newcommand{\hyperspace}{\text{Tem}_{+}}
\newcommand{\hypospace}{\text{Tem}_{-}}
\newcommand{\wlower}{w_{\Regionplus,f}^-}
\newcommand{\wupper}{w_{\Regionplus,f}^+}
\newcommand{\wsoln}{w_{\Regionplus,f}}
\newcommand{\parameasure}{\omega_{\Regionplus,p}}

% Fractal geometry notation
\newcommand{\tubezeta}{\widetilde\zeta}
\newcommand{\tubefn}{V_{X,\Omega}}
\newcommand{\partialzeta}{\widetilde\xi} 
\newcommand{\MinkContent}{\mathcal{M}^*}
\newcommand{\Mink}{\text{Mink}}
\newcommand{\dimension}{N}
\newcommand{\Cnr}{{C_{n,r}}}
\newcommand{\vkCurve}{{C'_{n,r}}}
\newcommand{\Knr}{{K_{n,r}}}
\newcommand{\Phinr}{{\Phi_{n,r}}}
\newcommand{\vkSnow}{{K'_{n,r}}}
\newcommand{\Mcontent}{\M_d^*}
\newcommand{\e}{\varepsilon}
\newcommand{\CantorSet}{\mathscr{C}_{\frac13}}
\DeclareMathOperator{\Cpt}{Cpt}
\newcommand{\measure}[1]{\left|#1\right|_\dimension}

\newcommand{\RRN}{\RR^\dimension}
\newcommand{\RRNplus}{\RR^{\dimension+1}}

%----------------------------------------------------------------------------------------------------------------

% My Operator Shortcuts
\renewcommand{\Re}{\text{Re}}
\renewcommand{\Im}{\text{Im}}
\DeclareMathOperator{\Res}{Res}
\providecommand{\supp}{\text{supp}}
\newcommand{\Id}{\text{id}}

% n^th commands
\renewcommand{\th}{^\text{th}}
\newcommand{\nth}{^\text{th}}

% Left-Right Pairings 
\newcommand{\enclose}[1]{\left(#1\right)}
\providecommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\suchthat}{\,\middle|\,} % For use within \set{}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

% Indicator Function
\RequirePackage{dsfont}
\newcommand{\1}{\mathds{1}}



%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%█..............................................................................................................█
%█................................................................................**............................█
%█...........................................................................***********........................█
%█..........................................................................************........................█
%█............................................................................*********.........................█
%█..................................................................*....*.************..*......................█
%█..........................................................*****..*.**************************.................█
%█..........................................................***************************************.*****.......█
%█...........................................................*******************************************........█
%█.....................................................***.********************************************.*.......█
%█.......................................................*************************************************......█
%█..................................................********************************************************....█
%█...................................................*****************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...........................*****************.....*******************************************************......█
%█........................***********************.*********************************************************.....█
%█........................***********************.********************************************************......█
%█..................****.********************************************************************************.......█
%█**************************************************************************************************............█
%█..................****.********************************************************************************.......█
%█........................***********************.********************************************************......█
%█........................***********************.*********************************************************.....█
%█...........................*****************.....*******************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...................................................*****************************************************......█
%█..................................................********************************************************....█
%█......................................................*************************************************.......█
%█....................................................***.********************************************.*........█
%█..........................................................*******************************************.........█
%█.........................................................***************************************.*****........█
%█.........................................................*****..*.**************************..................█
%█.................................................................*....*.************..*.......................█
%█...........................................................................*********..........................█
%█.........................................................................************.........................█
%█..........................................................................***********.........................█
%█...............................................................................**.............................█
%█..............................................................................................................█
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

==> commands/thesisCommands.tex <==
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%
%           ██╗    ██╗██╗██╗     ██╗         ██╗  ██╗ ██████╗ ███████╗███████╗███████╗██████╗
%           ██║    ██║██║██║     ██║         ██║  ██║██╔═══██╗██╔════╝██╔════╝██╔════╝██╔══██╗
%           ██║ █╗ ██║██║██║     ██║         ███████║██║   ██║█████╗  █████╗  █████╗  ██████╔╝
%           ██║███╗██║██║██║     ██║         ██╔══██║██║   ██║██╔══╝  ██╔══╝  ██╔══╝  ██╔══██╗
%           ╚███╔███╔╝██║███████╗███████╗    ██║  ██║╚██████╔╝██║     ██║     ███████╗██║  ██║
%            ╚══╝╚══╝ ╚═╝╚══════╝╚══════╝    ╚═╝  ╚═╝ ╚═════╝ ╚═╝     ╚═╝     ╚══════╝╚═╝  ╚═╝
%
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

\RequirePackage{amsmath}					% Useful package for math; already required by mathtools
\RequirePackage{amssymb}					% Needed for symbols such as \mathbb
\RequirePackage{mathrsfs} 					% Math script font

\usepackage[colorlinks=true,allcolors={blue}]{hyperref}

\usepackage[font={singlespacing},margin=1cm]{caption}
\usepackage[margin=0pt]{subfig}

\input{commands/letterCommands}
\input{commands/notation}
\input{commands/_thmSetupTCB.tex}



%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%█..............................................................................................................█
%█................................................................................**............................█
%█...........................................................................***********........................█
%█..........................................................................************........................█
%█............................................................................*********.........................█
%█..................................................................*....*.************..*......................█
%█..........................................................*****..*.**************************.................█
%█..........................................................***************************************.*****.......█
%█...........................................................*******************************************........█
%█.....................................................***.********************************************.*.......█
%█.......................................................*************************************************......█
%█..................................................********************************************************....█
%█...................................................*****************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...........................*****************.....*******************************************************......█
%█........................***********************.*********************************************************.....█
%█........................***********************.********************************************************......█
%█..................****.********************************************************************************.......█
%█**************************************************************************************************............█
%█..................****.********************************************************************************.......█
%█........................***********************.********************************************************......█
%█........................***********************.*********************************************************.....█
%█...........................*****************.....*******************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...................................................*****************************************************......█
%█..................................................********************************************************....█
%█......................................................*************************************************.......█
%█....................................................***.********************************************.*........█
%█..........................................................*******************************************.........█
%█.........................................................***************************************.*****........█
%█.........................................................*****..*.**************************..................█
%█.................................................................*....*.************..*.......................█
%█...........................................................................*********..........................█
%█.........................................................................************.........................█
%█..........................................................................***********.........................█
%█...............................................................................**.............................█
%█..............................................................................................................█
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
